A Unifying Framework for Some Directed Distances in Statistics

Density-based directed distances -- particularly known as divergences -- between probability distributions are widely used in statistics as well as in the adjacent research fields of information theory, artificial intelligence and machine learning. Prominent examples are the Kullback-Leibler information distance (relative entropy) which e.g. is closely connected to the omnipresent maximum likelihood estimation method, and Pearson's chisquare-distance which e.g. is used for the celebrated chisquare goodness-of-fit test. Another line of statistical inference is built upon distribution-function-based divergences such as e.g. the prominent (weighted versions of) Cramer-von Mises test statistics respectively Anderson-Darling test statistics which are frequently applied for goodness-of-fit investigations; some more recent methods deal with (other kinds of) cumulative paired divergences and closely related concepts. In this paper, we provide a general framework which covers in particular both the above-mentioned density-based and distribution-function-based divergence approaches; the dissimilarity of quantiles respectively of other statistical functionals will be included as well. From this framework, we structurally extract numerous classical and also state-of-the-art (including new) procedures. Furthermore, we deduce new concepts of dependence between random variables, as alternatives to the celebrated mutual information. Some variational representations are discussed, too.

==> COMP <==
#!/bin/bash
mf "\mode=ljfour; mag=1.2; input $1"; gftopk $1.720gf;
mf "\mode=ljfour; input $1"; gftopk $1.600gf;
 
mv *.tfm ../tfm; mv *pk ../pk; rm *gf; rm *.log;


==> COMPILE <==
#! /bin/bash
# blackboard typefaces by Anthony Phan.
# file: @compile (stupid compilation script)
# last modification: 09.08.2001.
# 
# This script is helful for me. I just type 'bash @compile'
# then drink my coffee. It produces metrics and bitmaps (pk)
# for the 'ljfour' mode, then it wipes out temporary files
# and put the useful stuff in some directory...
# PLEASE CHANGE THE THIS FILE FOR YOUR OWN NEEDS.

for xx in 17 12 10 9 8 7 6 5
do
    mf "\mode=ljfour; input mbb$xx"; gftopk mbb$xx.600gf;
    mf "\mode=ljfour; mag=1.2; input mbb$xx"; gftopk mbb$xx.720gf;
    mf "\mode=ljfour; input mbbx$xx"; gftopk mbbx$xx.600gf;
    mf "\mode=ljfour; mag=1.2; input mbbx$xx"; gftopk mbbx$xx.720gf;
done;

for fontxx in mbbheb10 mbbgr10 mbbi10 mbbsl10 mbbsc10 mbbr10 mbbcr10
do
    mf "\mode=ljfour; input $fontxx"; gftopk $fontxx.600gf;
    mf "\mode=ljfour; mag=1.2; input $fontxx"; gftopk $fontxx.720gf;
done;

mv *.tfm ../tfm; mv *pk ../pk; rm *gf; rm *.log;


